A Gibbs distribution that learns from GA dynamics

A general procedure of average-case performance evaluation for population dynamics such as genetic algorithms (GAs) is proposed and its validity is numerically examined. We introduce a learning algorithm of Gibbs distributions from training sets which are gene configurations (strings) generated by GA in order to figure out the statistical properties of GA from the view point of thermodynamics. The learning algorithm is constructed by means of minimization of the Kullback-Leibler information between a parametric Gibbs distribution and the empirical distribution of gene configurations. The formulation is applied to the solvable probabilistic models having multi-valley energy landscapes, namely, the spin glass chain and the Sherrington-Kirkpatrick model. By using computer simulations, we discuss the asymptotic behaviour of the effective temperature scheduling and the residual energy induced by the GA dynamics.

==> abstract.tex <==
\fontsize{9}{11}\selectfont 
A general procedure of 
average-case performance evaluation for 
population dynamics such as genetic algorithms (GAs) 
is proposed and its validity is numerically examined. 
We introduce a learning algorithm 
of Gibbs distributions 
from training sets which are 
gene configurations (strings) generated 
by GA in order to figure out 
the statistical properties of GA from 
the view point of thermodynamics. 
The learning algorithm is 
constructed by means of 
minimization of the 
Kullback-Leibler information between a parametric 
Gibbs distribution and the empirical distribution 
of gene configurations. 
The formulation is applied to 
the solvable probabilistic models 
having multi-valley energy landscapes, 
namely, the spin glass chain and 
the Sherrington-Kirkpatrick model. 
By using computer simulations, we discuss the asymptotic 
behaviour of the effective 
temperature scheduling and the residual energy induced by the GA dynamics. 


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Manabu Kitagata and Jun-ichi Inoue\\
  \fontsize{9}{11}\selectfont
  \textit{Complex Systems Engineering, Graduate School of Information Science and 
  Technology} \\ 
  \fontsize{9}{11}\selectfont
 \textit{Hokkaido University, N14-W9, Kita-ku, Sapporo 060-0814, Japan}\\
  \fontsize{9}{11}\selectfont
  \textit{kitagata@chaos1.complex.eng.hokudai.ac.jp, j\_inoue@complex.eng.hokudai.ac.jp}\\[12pt]
  %
  %\fontsize{11}{13}\selectfont
  %Third Author Name\\
  %\fontsize{9}{11}\selectfont
  %\textit{Department of Computing, Main University, MySecondTown, MyCountry}\\
  %\fontsize{9}{11}\selectfont
  %\textit{t\_author@xy.mu.edu}\\[12pt]
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont 
Genetic algorithms, 
Evolutionary optimization, 
Machine learning, 
Population dynamics, 
Thermodynamics, 
Average-case performance, 
Spin glass model, 
Statistical physics



==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{
A Gibbs distribution that learns from GA dynamics} 
%The Subtitle should have initial letters capitalized
%\fontsize{13}{15}\selectfont \textit{A procedure of evaluation for average-case performance of genetic algorithms}
}

